TensorSCONE: A Secure TensorFlow Framework using Intel SGX

Machine learning has become a critical component of modern data-driven online services. Typically, the training phase of machine learning techniques requires to process large-scale datasets which may contain private and sensitive information of customers. This imposes significant security risks since modern online services rely on cloud computing to store and process the sensitive data. In the untrusted computing infrastructure, security is becoming a paramount concern since the customers need to trust the thirdparty cloud provider. Unfortunately, this trust has been violated multiple times in the past. To overcome the potential security risks in the cloud, we answer the following research question: how to enable secure executions of machine learning computations in the untrusted infrastructure? To achieve this goal, we propose a hardware-assisted approach based on Trusted Execution Environments (TEEs), specifically Intel SGX, to enable secure execution of the machine learning computations over the private and sensitive datasets. More specifically, we propose a generic and secure machine learning framework based on Tensorflow, which enables secure execution of existing applications on the commodity untrusted infrastructure. In particular, we have built our system called TensorSCONE from ground-up by integrating TensorFlow with SCONE, a shielded execution framework based on Intel SGX. The main challenge of this work is to overcome the architectural limitations of Intel SGX in the context of building a secure TensorFlow system. Our evaluation shows that we achieve reasonable performance overheads while providing strong security properties with low TCB.

==> defs.tex <==
%% 
%% Functions
\newcommand{\timeOfTask}[1]{\ensuremath{t_T {#1} }}
\newcommand{\timeRead}[1]{\ensuremath{t_R {#1} }}
\newcommand{\timeWrite}[1]{\ensuremath{t_W {#1} }}


%% sets
\newcommand{\setFresh}{\mathcal{F}}
\newcommand{\setReused}{\mathcal{R}}


%% times
\newcommand{\timeHash}{\ensuremath{t_h}\xspace}
\newcommand{\timeMessage}{\ensuremath{t_m}\xspace}
\newcommand{\timeMemo}{\ensuremath{t_{memo}}\xspace}
\newcommand{\ninput}{\ensuremath{n_i}\xspace}
\newcommand{\noutput}{\ensuremath{n_O}\xspace}
\newcommand{\nmap}{\ensuremath{N_M}\xspace}
\newcommand{\nred}{\ensuremath{N_R}\xspace}
\newcommand{\ncon}{\ensuremath{N_C}\xspace}

\newcommand{\nkeysetmap}{\ensuremath{n_{mk}}}
\newcommand{\nkeyvaluemap}{\ensuremath{n_{m}}}
\newcommand{\nconAppend}{\ensuremath{H_{CA}}\xspace}
\newcommand{\nconFix}{\ensuremath{H_{CF}}\xspace}
\newcommand{\nconVariable}{\ensuremath{H_{CV}}\xspace}

%% numbers
\newcommand{\numberTasks}{\ensuremath{n_t}}
\newcommand{\inputSize}{\ensuremath{s_i}}
\newcommand{\avgChunkSize}{\ensuremath{s_c}}
\newcommand{\keyset}{\ensuremath{K}}


%% sizes
\newcommand{\sizeReducers}{\ensuremath{m_r}}



==> discussion.tex <==
\section{Discussion} 
\label{sec:discussion}
%
In this section, we want to judge the usefulness of TensorSCONE.
We focus on the comparison of TensorSCONE with other machine learning frameworks, as well as on the firmness of our security guarantees in practice.

\paragraph{Comparison of TensorSCONE with other machine learning frameworks}
Because of the nature of calculations in machine learning tasks, they can often be accelerated through parallel hardware.
\textit{GPU}s in particular offer speedups up to over one order of magnitude in theory compared to an all-purpose \textit{CPU}, and are regularly used in practical machine learning applications \cite{bekkerman2011scaling}.
Cloud vendors such as Google, Microsoft and Amazon advertise the availability of GPUs or other parallel hardware on machine learning specific cloud products \cite{machine_learning_aws,google_cloud_ml_engine,azure_machine_learning}.
Popular machine learning frameworks usually also offer GPU support, either in form of \textit{CUDA} support, or through more generic interfaces for parallel computing, such as \textit{openMP}.
\textit{Apache Singa}, \textit{torch}, \textit{Caffe} and TensorFlow are examples for this \cite{singa_gpu,torch_gpu,tensorflow_gpu,caffe_gpu}.

For TensorSCONE, we cannot offer support for GPUs or any computation hardware other than Intel CPUs that support SGX, because our security guarantees are realized by Intel SGX.
Training and classification times are therefore always several times longer with TensorSCONE compared to GPU implementations.
With the added overhead for security compared to pure CPU implementations, TensorSCONE is even less efficient, as we have found out in section \ref{sec:evaluation}.

On the other hand, we could not find a machine learning framework that offers the same degree of protection as TensorSCONE.
With data becoming more and more valuable, TensorSCONE fills a niche in the framework portfolio by offering high security guarantees that no other machine learning framework has.

\paragraph{Intel SGX vulnerabilities}
Since we use Intel SGX for protection, the security of TensorSCONE is subject to the same vulnerabilities that SGX is.
SGX has been the target of security researchers since its release.
Applications running in enclaves are vulnerable to the same type of side channel attacks as applications on normal CPUs are \cite{gotzfried2017cache}.
The particular types of side channel attacks mentioned by Götzfried et al. can be mitigated by the operating system or through microcode updates.
Since we do not trust the operating system in our threat model, SGX remains effected until the security holes are patched in hardware.
This will not be completed before the release of models past Intel's \textit{Cascade Lake} series \cite{whiskey_lake_vul_patches}.

Another vulnerability effecting Intel SGX specifically is \textit{Foreshadow} \cite{van2018foreshadow}.
Foreshadow leverages a bug in speculative execution to obtain the enclave's secret key.
It can be exploited by running only user software on the vulnerable machine, requiring no super user access.
It also allows manipulation of the attestation process, endangering both confidentiality and integrity of data in SGX enclaves.
While microcode updates can circumvent the exploit, we cannot trust the environment to have applied relevant updates.
Starting from \textit{Whiskey Lake} microarchitecture Intel CPUs, fixes in hardware will be included to prevent Foreshadow, but older CPUs supporting SGX will still be effected.

==> overview.tex <==
\section{Design}
\label{sec:overview}

%The main goal of our work is to provide \textit{TensorSCONE}, a framework for secure and privacy-preserving machine learning.
%In this section, we explore different design choices and explain the rationale for selecting the design choices we ultimately used.
%First, we give an overview by describing the threat model we design our protection for (\ref{sec:threat_model}) and explain our design goals (\ref{sec:design-goals}), then we explain the architecture of the resulting framework (\ref{sec:architecture}).
%
%
%%
%\subsection{Threat model} 
%\label{sec:threat_model}
%Generally, we use the same threat model as \textit{SGX} (\ref{sec:sgx-introduction}) and SCONE (\ref{sec:scone-overview}):
%We assume that the attacker has superuser access to operating system, and physical access to the hardware of the machines running the machine learning framework.
%This also allows the attacker to manipulate any network traffic from and to the machines.
%
%This scenario typically applies for cloud computing environments.
%The physical machine is shared by multiple tenants.
%The cloud provider and other tenants are possible attackers.
%Tenants are usually isolated through various means, but are ultimately out of control and must trust the isolation mechanisms employed by the cloud provider.
%Furthermore, staff of the cloud provider has hardware access to the machine.
%Cloud users must therefore trust the provider itself.
%In our threat model we do not trust the whole stack, including cloud provider, hardware, hypervisor, operating system and user software.

\myparagraph{Design goals} 
\label{sec:design-goals}

\paragraph{Confidentiality}
All data handled by the machine learning framework and the machine learning framework code itself may not be disclosed to or obtainable by an unauthorized party, which includes the cloud provider and other tenants.

\paragraph{Integrity}
Modifications on data handled by TensorSCONE that were done by an unauthorized party must be detectable and may not compromise internal state and functioning.

\paragraph{Transparency}
The secure machine learning framework must offer the same interface as the unprotected framework.
Graphs and training data must be usable in the same way.
Users do not have to change input data when switching from the unprotected to the protected framework.

\paragraph{Efficiency}
We aim to impose as little overhead as possible when adding security to the machine learning framework.
The user can decide to either run training and classification with full efficiency, or with added security and some overhead, which we will estimate.
We do not trade-off accuracy for security.
Accuracy will be the same as when using no protection.

\paragraph{Availability} We explicitly do not make guarantees on availability.
An attacker can easily deny access at any time given the access level mentioned in section \ref{sec:threat_model}.
Such failures must be detectable, however.


==> relatedwork.tex <==
\section{Related work} 
\label{sec:related-work}
%
Previous work has dealt with making machine learning more secure through other means than creating secure containers.
We present some solutions in section \ref{sec:machine_learning_on_encrypted_data}.
We want to find out the limitations of these approaches and see where improvement is needed.
There are also several other trusted execution frameworks that enable the usage of SGX without extensive change of the user application, which makes them potential candidates for usage in our work.
We did not consider ARM Trustzone\textregistered{} \cite{arm_trustzone} as an alternative \textit{TEE}, because it targets ARM processors, which are not commonly used in servers in data centers.


\subsection{Machine learning on randomized data} 
\label{sec:perturbed_mining}
%
Early work on preserving privacy for data mining techniques have relied on randomizing user data \cite{agrawal2000privacy,du2003using}.
These approaches trade of privacy for accuracy.
The work of Du et al. \cite{du2003using} includes a parameter that allows continuous choice between privacy and accuracy, having none of one, if the other is perfect.
The algorithms used aim to provide privacy preserving collection of data, and do not protect the results themselves in the cloud, nor do they protect the classification. 

\subsection{Machine learning on encrypted data} \label{sec:machine_learning_on_encrypted_data}
An approach reaching the same accuracy as unprotected variants is to perform machine learning on encrypted data.
Bost et al. \cite{bost2015machine} developed protocols to perform privacy preserving classification.
While this can protect the privacy of the users of a classification service, it does not cover training.
This approach does therefore only partially cover the goals for TensorSCONE.

Graepel et al. \cite{graepel2012ml} developed machine learning algorithms to perform both training and classification on encrypted data.
The solution is based on the properties of homomorphic encryption.
A homomorphic encryption scheme allows operations, such as multiplication and addition, on encrypted data, so that the result can be decrypted by the owner of the private key to yield the same as when performing the operation on the plaintext data.
%TODO maybe add a formular to show homomorphic encryption

The data owner first encrypts the training data with a homomorphic encryption scheme and then uploads it to a cloud provider.
The cloud provider then computes an encrypted model.
The model can then be downloaded by the data owner and used for classification.
For classification in the cloud, the data owner first encrypts the data to be classified and then uploads it to the cloud service hosting the encrypted model to classify the encrypted data, which yields an encrypted classification result.
The result is then downloaded and decrypted by the data owner. 
The cloud in this case is thought to be "honest but curious", that is, it correctly handles protocols and calculations, but is interested in obtaining information from data provided to it. 
This scheme does therefore not protect from an entirely malicious cloud that actively falsifies information.
The cloud user can test the fidelity of the cloud provider by requesting classifications of data that was used for training.
While the data itself might not be leaked, the provider for the calculations may cheat the agreement by using false coefficients that were easier to produce.
The main drawback of the solution proposed by Graepel et al. is however that the time required for classification and training is increased by six to seven orders of magnitude.
Thus the solution is not practical for secure machine learning in real world scenarios, where training a model may take weeks, even on hardware that is highly specialized for the machine learning task.

\subsection{SGX-based trusted execution frameworks}
%
In the next sections we want to present further frameworks that facilitate the usage of \textit{SGX}.
While they are possible alternatives for SCONE, we want to give reasons why we prefer SCONE.
%
%%
\subsubsection{Graphene}
%
Tsai et al. \cite{tsai2014cooperation} built the library \textit{OS} Graphene.
A library OS condenses all functionality of an operating system into a flat application library.
This library exposes system calls to the application, whereas it is using functionality of the host OS to serve the system calls to the application.
Depending on the implementation of the library OS, the interface between host OS and library OS is smaller and makes attacks from the containerized application to the host OS harder.
This allows the isolation of processes running under Graphene.

Similar to SCONE, Graphene uses a separate loader to bootstrap applications into the library OS.
Graphene also makes applications portable and easy to migrate, comparable to running inside a virtual machine, while having higher performance, because less OS features, like scheduler and memory management, are duplicated.

Graphene can also be compiled to support Intel SGX, which makes it an alternative for SCONE to consider.
A difference in the threat model between SCONE and Graphene is that Graphene generally trusts the host operating system.
Its use case lies in environments, where the host does not trust the applications it is running.
Another practical application for Graphene is the mutual isolation of applications running under it to minimize the effect of rogue applications.

Graphene applications still trust the results of system calls.
SCONE inverts that trust.
Applications that originally trust the OS are containerized with added SCONE runtime to protect it from the OS.
Graphene also does not have measures to speedup system calls that are inherently slow with SGX.
%
%%
\subsubsection{Rust SGX \textit{SDK}} 
%
Ding et al. \cite{ding2017poster} created an SDK for writing SGX enclave code in the Rust programming language.
The SDK builds on top of the Intel SGX SDK and reimplements Rust so that code can be directly compiled to SGX native machine code.
The Rust programming language offers strong security promises for memory and thread safety.
It can therefore mitigate exploitable implementation flaws in applications, which could lead to it getting compromised, even when running in a secure container.
The solution proposed by Ding et al. tackles the general problem that design flaws of the application running inside an enclave are not mitigated by SGX.
Applications need to be written in Rust, meaning existing C/C++ applications cannot be used.
We could not find deep learning frameworks implemented in Rust as of 2018.
%
%%
\subsubsection{Panoply}
%
In contrast to Graphene, Panoply is a framework that has the same goal as SCONE.
Panoply was presented by Shinde et al. in 2017 \cite{shinde2017panoply}.
Like SCONE, Panoply introduces a custom C library inside the SGX enclave.

A major design principle for Panoply was to reduce the trusted computing base, which is the code running inside the enclave, so that the framework is less prone to have exploitable bugs.
For this reason, the shim library simply exposes a \textit{POSIX} interface to the application and delegates all calls to the underlying operating system.
Results returned by the operating system are checked for malicious behavior.
The security checks are possible through explicit length statements for results in system calls.
When there are no boundaries given, such as for complex data structures, Panoply requires that the developer explicitly annotates the bounds inside the code using pragmas.

SCONE on the other hand does shift more functionality inside the enclave to avoid switching contexts.
Panoply also has no support for asynchronous system calls.
All system calls lead to synchronous enclave exits instead.

Panoply supports distributing processes and threads of an application over multiple SGX enclaves, what SCONE does not provide.
This distribution requires the developer to annotate the code to assign lines of code to different enclaves. 
An example for this can be seen in code snippet \ref{lst:panoply}.
%
\lstinputlisting[language=C,caption={Code from FreeTDS, annotated with Panoply pragmas (taken from \cite{shinde2017panoply})},label={lst:panoply}]{code_snippets/panoply.c}
%
The instructions of the OpenSSL interface on line 5 and 12 are surrounded by pragmas that cause Panoply to execute those instructions inside a different enclave called \texttt{privilege\_enclave}.
Based on those annotations, Panoply creates a dependency graph between the enclaves for data and control flow.
The shim library secures communication between enclaves transparently.
The channel is confidential, integrity protected and freshness of messages is guaranteed.
Sender and receiver are authenticated. 

Like SCONE, Panoply supports a dynamic number of application threads, compared to the static thread count when using plain SGX.
To make threads available to the application, Panoply implements the POSIX pthread \textit{API}.
Under the hood, each enclave of the application supports a fixed number of \texttt{k} threads by reserving SGX thread control blocks.
When a thread enters the enclave, the runtime first checks if the thread can be supported concurrently, that is, fewer than \texttt{k} threads are inside the same enclave.
If not, then Panoply spawns a new enclave to support another \texttt{k} threads.
Threads might need to access thread local memory of another thread that may reside inside another enclave and is thus protected from access.
As an alleviation, Panoply introduces a thread control manager that performs all shared memory operations for threads.
The application developer has to manually annotate variables that will be accessed concurrently.
The shim library may then redirect accesses to those annotated locations to the thread control manager, depending on whether another enclave was launched to support more threads.

Panoply does support \texttt{fork} and \texttt{exec}.
For \texttt{fork}, Panoply first creates a new untrusted child thread.
This new thread then creates and enters an enclave with the same code as the parent.
The semantics of \texttt{fork} require that the entire state of the parent is copied to the child process, which requires secure communication between parent and child enclave.
Panoply offers two strategies for the transfer.
It can either copy the entire state via the secure channel, or only areas that were manually annotated by the developer.

The performance of SCONE and Panoply based on the published papers is not directly comparable.
According to Shinde et al., Panoply adds an average \textit{CPU} overhead of 24\% for launching an enclave compared to the Intel SDK.
Benchmarks with the LMBench benchmarking framework yield that latency is increased by more than factor 3.
Finally, the throughput when serving static web pages with the H2O web server becomes increasingly smaller with the size of the web page.
It reaches about 25\% of the throughput of the original application without Panoply when serving 6 \textit{KB} pages.

Panoply and SCONE have similar goals, but different strategies. Moreover, Panoply requires the developer to annotate their code at the level of a single line of code, which makes it a greater effort to port an application to Panoply.
Like SCONE, Panoply does not mitigate denial-of-service attacks, bugs in the application itself, side channel attacks on enclaves and bugs in SGX.

==> space-tricks.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}

%\usepackage[small,compact,noindentafter]{titlesec}
%\usepackage[compact]{titlesec}
%
%\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}
%
\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

%\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}

